Detecting unusual input to neural networks

Evaluating a neural network on an input that differs markedly from the training data might cause erratic and flawed predictions. We study a method that judges the unusualness of an input by evaluating its informative content compared to the learned parameters. This technique can be used to judge whether a network is suitable for processing a certain input and to raise a red flag that unexpected behavior might lie ahead. We compare our approach to various methods for uncertainty evaluation from the literature for various datasets and scenarios. Specifically, we introduce a simple, effective method that allows to directly compare the output of such metrics for single input points even if these metrics live on different scales.

==> pics_copy <==
sed -nE 's/.*\\includegraphics\[.*\]\{(.*)\}.*/\1/p' arxiv_unexpected.tex | sed 's/.pdf$//' | sed  -E 's/^(.*)$/..\/..\/\1.pdf/' | sed 's/[{}]//g' | xargs -I {} cp {} .

